On Applying Meta-path for Network Embedding in Mining Heterogeneous DBLP Network

In recent time, applications of network embedding in mining real-world information network have been widely reported in the literature. Majority of the information networks are heterogeneous in nature. Meta-path is one of the popularly used approaches for generating embedding in heterogeneous networks. As meta-path guides the models towards a specific sub-structure, it tends to lose some hetero- geneous characteristics inherently present in the underlying network. In this paper, we systematically study the effects of different meta-paths using different state-of-art network embedding methods (Metapath2vec, Node2vec, and VERSE) over DBLP bibliographic network and evaluate the performance of embeddings using two applications (co-authorship prediction and authors research area classification tasks). From various experimental observations, it is evident that embedding using different meta-paths perform differently over different tasks. It shows that meta- paths are task-dependent and can not be generalized for different tasks. We further observe that embedding obtained after considering all the node and relation types in bibliographic network outperforms its meta- path based counterparts.

==> table/auc_all.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
\caption{AUC score for Co-Authorship Prediction}
\label{tab:auc_all}
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\% \\ Training\\ Data\end{tabular}}} & \multicolumn{4}{c|}{\textbf{MetaPath2vec}}   & \multicolumn{4}{c|}{\textbf{Node2vec}}       & \multicolumn{4}{c|}{\textbf{VERSE}}          \\ \cline{2-13} 
                                                                                     & \textbf{\begin{tabular}[c]{@{}c@{}}DBLP-\\AVA\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}DBLP-\\APA\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}DBLP-\\AA\end{tabular}}  & \textbf{\begin{tabular}[c]{@{}c@{}}DBLP-\\All\end{tabular}}   & \textbf{\begin{tabular}[c]{@{}c@{}}DBLP-\\AVA\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}DBLP-\\APA\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}DBLP-\\AA\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}DBLP-\\All\end{tabular}}   & \textbf{\begin{tabular}[c]{@{}c@{}}DBLP-\\AVA\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}DBLP-\\APA\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}DBLP-\\AA\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}DBLP-\\All\end{tabular}}   \\ \hline
\textbf{5}                                                                        & 0.728          & 0.724  &    & \textbf{0.756} & 0.741        & 0.756 &      & \textbf{0.768} & 0.752        & 0.772 &      & \textbf{0.790} \\ \hline
\textbf{10}                                                                         & 0.733        & 0.730  &    & \textbf{0.761} & 0.745        & 0.762 &      & \textbf{0.773} & 0.757        & 0.778 &      & \textbf{0.794} \\ \hline
\textbf{20}                                                                         & 0.735        & 0.734  &    & \textbf{0.764} & 0.748        & 0.764 &      & \textbf{0.774} & 0.761        & 0.782 &      & \textbf{0.796} \\ \hline
\textbf{30}                                                                         & 0.736        & 0.734  &    & \textbf{0.765} & 0.749        & 0.764 &      & \textbf{0.775} & 0.761        & 0.783 &      & \textbf{0.797} \\ \hline
\textbf{40}                                                                         & 0.737        & 0.736  &    & \textbf{0.766} & 0.749        & 0.765 &      & \textbf{0.777} & 0.762        & 0.784 &      & \textbf{0.796} \\ \hline
\textbf{50}                                                                         & 0.737        & 0.736  &    & \textbf{0.765} & 0.749        & 0.765 &      & \textbf{0.777} & 0.762        & 0.784 &      & \textbf{0.797} \\ \hline
\textbf{60}                                                                         & 0.736        & 0.736  &    & \textbf{0.767} & 0.750        & 0.766 &      & \textbf{0.775} & 0.762        & 0.785 &      & \textbf{0.797} \\ \hline 
\textbf{70}                                                                         & 0.737        & 0.738  &    & \textbf{0.765} & 0.750        & 0.766 &      & \textbf{0.777} & 0.761        & 0.785 &      & \textbf{0.797} \\ \hline
\textbf{80}                                                                         & 0.738        & 0.739  &    & \textbf{0.766} & 0.750        & 0.766 &      & \textbf{0.777} & 0.764        & 0.784 &      & \textbf{0.796} \\ \hline
\textbf{90}                                                                         & 0.737        & 0.736  &    & \textbf{0.766} & 0.749        & 0.766 &      & \textbf{0.775} & 0.765        & 0.784 &      & \textbf{0.797} \\ \hline
\end{tabular}
}
\end{table*}


==> table/auc_all_new.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
\caption{AUC score for Co-Authorship Prediction}
\label{tab:auc_all}
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\%\\ Training\\ Data\end{tabular}}} & \multicolumn{4}{c|}{\textbf{MetaPath2vec}}                                                                                                                                                                                                               & \multicolumn{4}{c|}{\textbf{Node2vec}}                                                                                                                                                                                                                   & \multicolumn{4}{c|}{\textbf{VERSE}}                                                                                                                                                                                                                      \\ \cline{2-13} 
                                                                                       & \textbf{\begin{tabular}[c]{@{}c@{}}DBLP-\\ ACA\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}DBLP-\\ APA\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}DBLP-\\ AA\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}DBLP-\\ All\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}DBLP-\\ ACA\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}DBLP-\\ APA\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}DBLP-\\ AA\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}DBLP-\\ All\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}DBLP-\\ ACA\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}DBLP-\\ APA\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}DBLP-\\ AA\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}DBLP-\\ All\end{tabular}} \\ \hline
\textbf{0.05}  & 0.728        & 0.724 & 0.722 & \textbf{0.756} & 0.741    & 0.756 & 0.76  & \textbf{0.768} & 0.752 & 0.772 & 0.775 & \textbf{0.79}  \\
\textbf{0.1}   & 0.733        & 0.73  & 0.728 & \textbf{0.761} & 0.745    & 0.762 & 0.766 & \textbf{0.773} & 0.757 & 0.778 & 0.781 & \textbf{0.794} \\
\textbf{0.2}   & 0.735        & 0.734 & 0.732 & \textbf{0.764} & 0.748    & 0.764 & 0.77  & \textbf{0.774} & 0.761 & 0.782 & 0.785 & \textbf{0.796} \\
\textbf{0.3}   & 0.736        & 0.734 & 0.733 & \textbf{0.765} & 0.749    & 0.764 & 0.77  & \textbf{0.775} & 0.761 & 0.783 & 0.787 & \textbf{0.797} \\
\textbf{0.4}   & 0.737        & 0.736 & 0.734 & \textbf{0.766} & 0.749    & 0.765 & 0.771 & \textbf{0.777} & 0.762 & 0.784 & 0.786 & \textbf{0.796} \\
\textbf{0.5}   & 0.737        & 0.736 & 0.734 & \textbf{0.765} & 0.749    & 0.765 & 0.771 & \textbf{0.777} & 0.762 & 0.784 & 0.787 & \textbf{0.797} \\
\textbf{0.6}   & 0.736        & 0.736 & 0.735 & \textbf{0.767} & 0.75     & 0.766 & 0.771 & \textbf{0.775} & 0.762 & 0.785 & 0.787 & \textbf{0.797} \\
\textbf{0.7}   & 0.737        & 0.738 & 0.734 & \textbf{0.765} & 0.75     & 0.766 & 0.773 & \textbf{0.777} & 0.761 & 0.785 & 0.787 & \textbf{0.797} \\
\textbf{0.8}   & 0.738        & 0.739 & 0.736 & \textbf{0.766} & 0.75     & 0.766 & 0.773 & \textbf{0.777} & 0.764 & 0.784 & 0.788 & \textbf{0.796} \\
\textbf{0.9}   & 0.737        & 0.736 & 0.741 & \textbf{0.766} & 0.749    & 0.766 & 0.773 & \textbf{0.775} & 0.765 & 0.784 & 0.786 & \textbf{0.797} \\ \hline
\end{tabular}
}
\end{table*}


==> table/auc_new.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{Prediction Performance}
\label{tab:result}
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|||c|c|c|}
\hline
\multirow{2}{*}{Network} & \multicolumn{3}{c|||}{\textbf{AUC score for Co-authorsip Prediction}} & \multicolumn{3}{c|}{\textbf{Accuracy for Author's Multiclass Classification}} \\ \cline{2-7} 
                         & Metapath2vec          & Node2vec             & VERSE                & Metapath2vec              & Node2vec             & VERSE                      \\ \hline
DBLP-AA                  & 0.736                 & 0.773                & 0.788                &  0.504                         & 0.486                & 0.536                      \\ \hline
DBLP-APA                 & 0.739                 & 0.766                & 0.784                &    0.539                       & 0.544                & 0.531                      \\ \hline
DBLP-AVA                 & 0.738                 & 0.75                 & 0.764                & 0.565                     & {\bf 0.559}                & 0.605                      \\ \hline
DBLP-All                 & \textbf{0.766}        & \textbf{0.777}       & \textbf{0.796}       &     {\bf 0.566}                      &   0.555                   & \textbf{0.624}             \\ \hline
\end{tabular}
}
\end{table}

